Condition Monitoring with Machine Learning: A Data-Driven Framework for Quantifying Wind Turbine Energy Loss

Wind energy significantly contributes to the global shift towards renewable energy, yet operational challenges, such as Leading-Edge Erosion on wind turbine blades, notably reduce energy output. This study introduces an advanced, scalable machine learning framework for condition monitoring of wind turbines, specifically targeting improved detection of anomalies using Supervisory Control and Data Acquisition data. The framework effectively isolates normal turbine behavior through rigorous preprocessing, incorporating domain-specific rules and anomaly detection filters, including Gaussian Mixture Models and a predictive power score. The data cleaning and feature selection process enables identification of deviations indicative of performance degradation, facilitating estimates of annual energy production losses. The data preprocessing methods resulted in significant data reduction, retaining on average 31% of the original SCADA data per wind farm. Notably, 24 out of 35 turbines exhibited clear performance declines. At the same time, seven improved, and four showed no significant changes when employing the power curve feature set, which consisted of wind speed and ambient temperature. Models such as Random Forest, XGBoost, and KNN consistently captured subtle but persistent declines in turbine performance. The developed framework provides a novel approach to existing condition monitoring methodologies by isolating normal operational data and estimating annual energy loss, which can be a key part in reducing maintenance expenditures and mitigating economic impacts from turbine downtime.

==> Bibliography/Bibliography.tex <==
% References section

% can use a bibliography generated by BibTeX as a .bbl file
% BibTeX documentation can be easily obtained at:
% http://mirror.ctan.org/biblio/bibtex/contrib/doc/
% The IEEEtran BibTeX style support page is at:
% http://www.michaelshell.org/tex/ieeetran/bibtex/
%\bibliographystyle{IEEEtran}
% argument is your BibTeX string definitions and bibliography database(s)
%\bibliography{IEEEabrv,../bib/paper}
%

% <OR> manually copy in the resultant .bbl file (THIS IS WHAT WE DO)
% set second argument of \begin to the number of references
% (used to reserve space for the reference number labels box)


https://sdgs.un.org/goals


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Real Bib
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
@misc{EUWind,
    author = "European Commission",
    title = "An EU Strategy to harness the potential of offshore renewable energy for a climate neutral future",
    url = "https://eur-lex.europa.eu/legal-content/EN/TXT/?uri=celex:52020DC0741",
    urldate = "2025-05-21"
}


@misc{IRENA,
    author = "International Renewable Energy Agency",
    title = "Reneable Power Generation Costs in 2019",
    url = "https://www.irena.org/-/media/Files/IRENA/Agency/Publication/2020/Jun/IRENA_Power_Generation_Costs_2019.pdf",
    urldate = "2025-05-21"
}

@inproceedings{bonacina2022use,
  title={On the use of artificial intelligence for condition monitoring in horizontal-axis wind turbines},
  author={Bonacina, Fabrizio and Miele, Eric Stefan and Corsini, Alessandro},
  booktitle={IOP Conference Series: Earth and Environmental Science},
  volume={1073},
  number={1},
  pages={012005},
  year={2022},
  organization={IOP Publishing}
}

@article{meyer2021multi,
  title={Multi-target normal behaviour models for wind farm condition monitoring},
  author={Meyer, Angela},
  journal={Applied Energy},
  volume={300},
  pages={117342},
  year={2021},
  publisher={Elsevier}
}

@article{wang2014copula,
  title={Copula-based model for wind turbine power curve outlier rejection},
  author={Wang, Yue and Infield, David G and Stephen, Bruce and Galloway, Stuart J},
  journal={Wind Energy},
  volume={17},
  number={11},
  pages={1677--1688},
  year={2014},
  publisher={Wiley Online Library}
}

@inproceedings{yasuda2017system,
  title={System health monitoring of wind turbines using SCADA data and gaussian mixture models},
  author={Yasuda, Akihisa and Ogata, Jun and Murakawa, Masahiro and Morikawa, Hiroyuki and Iida, Makoto},
  booktitle={PHM Society Asia-Pacific Conference},
  volume={1},
  number={1},
  year={2017}
}

@inproceedings{papatheou2014wind,
  title={Wind turbine structural health monitoring: a short investigation based on SCADA data},
  author={Papatheou, Evangelos and Dervilis, Nikolaos and Maguire, Eoghan and Worden, Keith},
  booktitle={EWSHM-7th European Workshop on Structural Health Monitoring},
  year={2014}
}

@inproceedings{chesterman2021condition,
  title={Condition monitoring of wind turbines and extraction of healthy training data using an ensemble of advanced statistical anomaly detection models},
  author={Chesterman, Xavier and Verstraeten, Timothy and Daems, Pieter-Jan and Now{\'e}, Ann and Helsen, Jan},
  booktitle={Annual Conference of the PHM Society},
  volume={13},
  number={1},
  year={2021}
}

@inproceedings{bilendo2021intelligent,
  title={An intelligent data-driven machine learning approach for fault detection of wind turbines},
  author={Bilendo, Francisco and Badihi, Hamed and Lu, Ningyun and Cambron, Philippe and Jiang, Bin},
  booktitle={2021 6th International Conference on Power and Renewable Energy (ICPRE)},
  pages={444--449},
  year={2021},
  organization={IEEE}
}

@article{jin2022condition,
  title={Condition monitoring of wind turbine generator based on transfer learning and one-class classifier},
  author={Jin, Xiaohang and Pan, Hengtuo and Ying, Chengzuo and Kong, Ziqian and Xu, Zhengguo and Zhang, Bin},
  journal={IEEE Sensors Journal},
  volume={22},
  number={24},
  pages={24130--24139},
  year={2022},
  publisher={IEEE}
}

@article{izquierdo2019framework,
  title={Framework for managing maintenance of wind farms based on a clustering approach and dynamic opportunistic maintenance},
  author={Izquierdo, Juan and Crespo M{\'a}rquez, Adolfo and Uribetxebarria, Jone and Erguido, Asier},
  journal={Energies},
  volume={12},
  number={11},
  pages={2036},
  year={2019},
  publisher={MDPI}
}

@article{oliveira2024wind,
  title={Wind turbine SCADA data imbalance: A review of its impact on health condition analyses and mitigation strategies},
  author={Oliveira-Filho, Adaiton and Comeau, Monelle and Cave, James and Nasr, Charbel and C{\^o}t{\'e}, Pavel and Tahan, Antoine},
  journal={Energies},
  volume={18},
  number={1},
  pages={59},
  year={2024},
  publisher={MDPI}
}

@inproceedings{meyer2020data,
  title={Data-driven performance fault detection in commercial wind turbines},
  author={Meyer, Angela and Brodbeck, Bernhard},
  booktitle={PHM Society European Conference},
  volume={5},
  number={1},
  pages={7--7},
  year={2020}
}

@article{cappugi2021machine,
  title={Machine learning-enabled prediction of wind turbine energy yield losses due to general blade leading edge erosion},
  author={Cappugi, Lorenzo and Castorrini, Alessio and Bonfiglioli, Aldo and Minisci, Edmondo and Campobasso, M Sergio},
  journal={Energy Conversion and Management},
  volume={245},
  pages={114567},
  year={2021},
  publisher={Elsevier}
}

@article{duthe2021modeling,
  title={Modeling and monitoring erosion of the leading edge of wind turbine blades},
  author={Duth{\'e}, Gregory and Abdallah, Imad and Barber, Sarah and Chatzi, Eleni},
  journal={Energies},
  volume={14},
  number={21},
  pages={7262},
  year={2021},
  publisher={MDPI}
}

@article{visbech2023introducing,
  title={Introducing a data-driven approach to predict site-specific leading-edge erosion from mesoscale weather simulations},
  author={Visbech, Jens and G{\"o}{\c{c}}men, Tuhfe and Hasager, Charlotte Bay and Shkalov, Hristo and Handberg, Morten and Nielsen, Kristian Pagh},
  journal={Wind Energy Science},
  volume={8},
  number={2},
  pages={173--191},
  year={2023},
  publisher={Copernicus Publications G{\"o}ttingen, Germany}
}

@inproceedings{castorrini2024opensource,
  title={Opensource machine learning metamodels for assessing blade performance impairment due to general leading edge degradation},
  author={Castorrini, A and Ortolani, A and Minisci, E and Campobasso, MS},
  booktitle={Journal of Physics: Conference Series},
  volume={2767},
  number={5},
  pages={052055},
  year={2024},
  organization={IOP Publishing}
}

@techreport{ehrmann2017effect,
  title={Effect of surface roughness on wind turbine performance},
  author={Ehrmann, Robert S and Wilcox, Benjamin and White, Edward B and Maniaci, David Charles},
  year={2017},
  institution={Sandia National Lab.(SNL-NM), Albuquerque, NM (United States)}
}

@article{sareen2014effects,
  title={Effects of leading edge erosion on wind turbine blade performance},
  author={Sareen, Agrim and Sapre, Chinmay A and Selig, Michael S},
  journal={Wind energy},
  volume={17},
  number={10},
  pages={1531--1542},
  year={2014},
  publisher={Wiley Online Library}
}

@inproceedings{bak2020influence,
  title={The influence of leading edge roughness, rotor control and wind climate on the loss in energy production},
  author={Bak, Christian and Forsting, Alexander M and Sorensen, Niels N},
  booktitle={Journal of Physics: Conference Series},
  volume={1618},
  number={5},
  pages={052050},
  year={2020},
  organization={IOP Publishing}
}

@inproceedings{kruse2018predicting,
  title={Predicting the Influence of Surface Protuberance on the Aerodynamic Characteristics of a NACA 633-418},
  author={Kruse, Emil Krog and S{\o}rensen, Niels N and Bak, Christian},
  booktitle={Journal of Physics: Conference Series},
  volume={1037},
  number={2},
  pages={022008},
  year={2018},
  organization={IOP Publishing}
}

@article{schramm2017influence,
  title={The influence of eroded blades on wind turbine performance using numerical simulations},
  author={Schramm, Matthias and Rahimi, Hamid and Stoevesandt, Bernhard and Tangager, Kim},
  journal={Energies},
  volume={10},
  number={9},
  pages={1420},
  year={2017},
  publisher={MDPI}
}

@thesis{VUGS_AND_BUCH_TO_THE_TOP,
    title={A Data-Driven Approach for Evaluating Annual
    Energy Production Loss Using Wind Turbine
    SCADA Data.},
    author={Buchberg, Emil Marcus and Nielsen, Kent Vugs},
    year={2024},
    school    = {Aalborg University},
    type      = {kandidatprojekt}        
}


@inproceedings{ozccakmak2024determination,
  title={Determination of annual energy production loss due to erosion on wind turbine blades},
  author={{\"O}z{\c{c}}akmak, {\"O}zge Sinem and Bretos, David and M{\'e}ndez, Beatriz and Bak, Christian},
  booktitle={Journal of Physics: Conference Series},
  volume={2767},
  number={2},
  pages={022066},
  year={2024},
  organization={IOP Publishing}
}

@article{morrison2022anomaly,
  title={Anomaly detection in wind turbine SCADA data for power curve cleaning},
  author={Morrison, Rory and Liu, Xiaolei and Lin, Zi},
  journal={Renewable Energy},
  volume={184},
  pages={473--486},
  year={2022},
  publisher={Elsevier}
}

@article{chesterman2023overview,
  title={Overview of normal behavior modeling approaches for SCADA-based wind turbine condition monitoring},
  author={Chesterman, Xavier and Verstraeten, Timothy and Daems, Pieter-Jan and Nowé, Ann and Helsen, Jan},
  journal={Wind Energy Science},
  volume={8},
  pages={893--914},
  year={2023},
  publisher={Copernicus GmbH},
  doi={10.5194/wes-8-893-2023},
}

@article{pandit2022scada,
  title={SCADA data for wind turbine data-driven condition/performance monitoring: A review on state-of-art, challenges and future trends},
  author={Pandit, Ravi and Astolfi, Davide and Hong, Jiarong and Infield, David and Santos, Matilde},
  journal={Wind Engineering},
  volume={47},
  number={2},
  pages={422--441},
  year={2022},
  publisher={SAGE Publications},
  doi={10.1177/0309524X221124031}
}

@article{panthi2023quantification,
  title={Quantification of wind turbine energy loss due to leading-edge erosion through infrared-camera imaging, numerical simulations, and assessment against SCADA and meteorological data},
  author={Panthi, Keshav and Iungo, Giacomo Valerio},
  journal={Wind Energy},
  volume={26},
  number={3},
  pages={266--282},
  year={2023},
  publisher={Wiley Online Library}
}

@article{Byrne2020,
  author    = {Raymond Byrne and Davide Astolfi and Francesco Castellani and Neil J. Hewitt},
  title     = {A Study of Wind Turbine Performance Decline with Age through Operation Data Analysis},
  journal   = {Energies},
  volume    = {13},
  number    = {8},
  pages     = {2086},
  year      = {2020},
  publisher = {MDPI},
  doi       = {10.3390/en13082086},
}

@article{Astolfi2022,
  author    = {Davide Astolfi and Ravi Pandit and Ludovica Celesti and Matteo Vedovelli and Andrea Lombardi and Ludovico Terzi},
  title     = {Data-Driven Assessment of Wind Turbine Performance Decline with Age and Interpretation Based on Comparative Test Case Analysis},
  journal   = {Sensors},
  volume    = {22},
  number    = {9},
  pages     = {3180},
  year      = {2022},
  publisher = {MDPI},
  doi       = {10.3390/s22093180}
}

@inproceedings{mathew2022estimation,
  author    = {Mathew, M.S. and Kandukuri, S.T. and Omlin, C.W.},
  title     = {Estimation of Wind Turbine Performance Degradation with Deep Neural Networks},
  booktitle = {PHM Society European Conference},
  year      = {2022},
  volume    = {7},
  number    = {1},
  pages     = {351--359},
  month     = jun,
  doi       = {10.36001/phme.2022.v7i1.3328}
}

@inproceedings{barnabei2024nbm,
  author    = {Valerio F. Barnabei and Filippo De Girolamo and Tullio C. M. Ancora and Lorenzo Tieghi and Giovanni Delibra and Alessandro Corsini},
  title     = {Normal Behaviour Modeling of HAWT Fleets Using SCADA-Based Feature Engineering},
  booktitle = {Proceedings of Global Power and Propulsion Society (GPPS Chania24)},
  year      = {2024},
  organization = {Global Power and Propulsion Society}
}

@article{bilendo2023applications,
  author    = {Francisco Bilendo and Angela Meyer and Hamed Badihi and Ningyun Lu and Philippe Cambron and Bin Jiang},
  title     = {Applications and Modeling Techniques of Wind Turbine Power Curve for Wind Farms—A Review},
  journal   = {Energies},
  volume    = {16},
  number    = {1},
  pages     = {180},
  year      = {2023},
  publisher = {MDPI},
  doi       = {10.3390/en16010180},
}

@article{Astolfi2021V52Aging,
  author    = {Davide Astolfi and Raymond Byrne and Francesco Castellani},
  title     = {Estimation of the Performance Aging of the Vestas V52 Wind Turbine through Comparative Test Case Analysis},
  journal   = {Energies},
  volume    = {14},
  number    = {4},
  pages     = {915},
  year      = {2021},
  publisher = {MDPI},
  doi       = {10.3390/en14040915},
}

@article{chandola2009anomaly,
  title={Anomaly detection: A survey},
  author={Chandola, Varun and Banerjee, Arindam and Kumar, Vipin},
  journal={ACM computing surveys (CSUR)},
  volume={41},
  number={3},
  pages={1--58},
  year={2009},
  publisher={ACM New York, NY, USA}
}

@article{lin2020wind,
  title={Wind power prediction based on high-frequency SCADA data along with isolation forest and deep learning neural networks},
  author={Lin, Zi and Liu, Xiaolei and Collu, Maurizio},
  journal={International Journal of Electrical Power \& Energy Systems},
  volume={118},
  pages={105835},
  year={2020},
  publisher={Elsevier}
}

@inproceedings{Miele2022,
  author       = {Eric Stefan Miele and Fabrizio Bonacina and Alessandro Corsini and Arianna Peruch and Marco Cannarozzo and Daniele Baldan and Francesco Pennisi},
  title        = {Unsupervised Feature Selection of Multi-Sensor SCADA Data in Horizontal Axis Wind Turbine Condition Monitoring},
  booktitle    = {Proceedings of the ASME Turbo Expo 2022: Turbomachinery Technical Conference and Exposition},
  year         = {2022},
  volume       = {11},
  number       = {V011T38A015},
  doi          = {10.1115/GT2022-82462},
  publisher    = {American Society of Mechanical Engineers},
}

@software{wetschoreck_krabel_krishnamurthy_2020,
  author       = {Wetschoreck, Florian and Krabel, Tobias and Krishnamurthy, Surya},
  title        = {8080labs/ppscore: zenodo release (Version 1.1.2)},
  year         = {2020},
  publisher    = {Zenodo},
  doi          = {10.5281/zenodo.4091345},
  url          = {https://doi.org/10.5281/zenodo.4091345}
}

@book{bishop2007,
  author = {Bishop, Christopher M.},
  edition = 1,
  isbn = {0387310738},
  publisher = {Springer},
  title = {Pattern Recognition and Machine Learning (Information Science and Statistics)},
  year = 2007
}

@misc{holbert_mahalanobis_2021,
  author       = {C. F. Holbert},
  title        = {Outlier Detection with Mahalanobis Distance},
  year         = {2021},
  url          = {https://www.cfholbert.com/blog/outlier_mahalanobis_distance/},
  note         = {Accessed: 2025-05-24},
}

@book{Hastie2009,
  title     = {The Elements of Statistical Learning: Data Mining, Inference, and Prediction},
  author    = {Trevor Hastie and Robert Tibshirani and Jerome Friedman},
  year      = {2009},
  edition   = {2},
  publisher = {Springer},
  isbn      = {978-0-387-84858-7},
}

@article{geurts2006extremely,
  title={Extremely randomized trees},
  author={Geurts, Pierre and Ernst, Damien and Wehenkel, Louis},
  journal={Machine learning},
  volume={63},
  number={1},
  pages={3--42},
  year={2006},
  publisher={Springer}
}

@article{scikit-learn,
  title={Scikit-learn: Machine Learning in Python},
  author={Pedregosa, Fabian and Varoquaux, Ga{\"e}l and Gramfort, Alexandre and Michel, Vincent and Thirion, Bertrand and Grisel, Olivier and Blondel, Mathieu and Prettenhofer, Peter and Weiss, Ron and Dubourg, Vincent and Vanderplas, Jake and Passos, Alexandre and Cournapeau, David and Brucher, Matthieu and Perrot, Matthieu and Duchesnay, {\'E}douard},
  journal={Journal of Machine Learning Research},
  volume={12},
  pages={2825--2830},
  year={2011}
}

@article{Janssens2016,
  title     = {Data-driven multivariate power curve modeling of offshore wind turbines},
  author    = {Olivier Janssens and Nymfa Noppe and Christof Devriendt and Rik Van de Walle and Sofie Van Hoecke},
  journal   = {Engineering Applications of Artificial Intelligence},
  volume    = {55},
  pages     = {331--338},
  year      = {2016},
  publisher = {Elsevier},
  doi       = {10.1016/j.engappai.2016.08.003},
}

@article{gill2011wind,
  title={Wind turbine condition assessment through power curve copula modeling},
  author={Gill, Simon and Stephen, Bruce and Galloway, Stuart},
  journal={IEEE Transactions on Sustainable Energy},
  volume={3},
  number={1},
  pages={94--101},
  year={2011},
  publisher={IEEE}
}

@article{lyons2021applied,
  title={Applied machine learning techniques for performance analysis in large wind farms},
  author={Lyons, John Thomas and G{\"o}{\c{c}}men, Tuhfe},
  journal={Energies},
  volume={14},
  number={13},
  pages={3756},
  year={2021},
  publisher={MDPI}
}

@book{Goodfellow-et-al-2016,
  title     = {Deep Learning},
  author    = {Ian Goodfellow and Yoshua Bengio and Aaron Courville},
  publisher = {MIT Press},
  year      = {2016},
  note      = {\url{http://www.deeplearningbook.org}}
}

@misc{XGBoost_doc,
    title = "XGBoost documentation: Introduction to Boosted Trees",
    url = "https://xgboost.readthedocs.io/en/stable/index.html",
    urldate = "2024-12-17"
}

@article{singh2022scada,
  title={SCADA system dataset exploration and machine learning based forecast for wind turbines},
  author={Singh, Upma and Rizwan, M},
  journal={Results in Engineering},
  volume={16},
  pages={100640},
  year={2022},
  publisher={Elsevier}
}
@inproceedings{xgboost,
 author = {Chen, Tianqi and Guestrin, Carlos},
 title = {{XGBoost}: A Scalable Tree Boosting System},
 booktitle = {Proceedings of the 22nd ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
 series = {KDD '16},
 year = {2016},
 isbn = {978-1-4503-4232-2},
 location = {San Francisco, California, USA},
 pages = {785--794},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/2939672.2939785},
 acmid = {2939785},
 publisher = {ACM},
}

@misc{wikipedia_mahalanobis,
  author       = "{Wikipedia contributors}",
  title        = "{Mahalanobis distance --- Wikipedia{,} The Free Encyclopedia}",
  year         = "2025",
  url          = "https://en.wikipedia.org/wiki/Mahalanobis_distance",
  note         = "[Online; accessed 26-May-2025]"
}
@misc{cansiz2021multivariate,
  author       = {Sergen Cansiz},
  title        = {Multivariate Outlier Detection in Python},
  year         = {2021},
  howpublished = {\url{https://medium.com/data-science/multivariate-outlier-detection-in-python-e946cfc843b3}},
  note         = {[Online; accessed 26-May-2025]}
}

@article{breiman2001random,
  title        = {Random Forests},
  author       = {Breiman, Leo},
  journal      = {Machine Learning},
  volume       = {45},
  number       = {1},
  pages        = {5--32},
  year         = {2001},
  publisher    = {Springer},
  doi          = {10.1023/A:1010933404324},
}

@misc{wikipedia_box_plot,
  author       = {{Wikipedia contributors}},
  title        = {Box plot},
  year         = {2025},
  month        = {May},
  note         = {Accessed on 2025-05-28},
  url          = {https://en.wikipedia.org/wiki/Box_plot}
}

@article{hewamalage2023forecast,
  title={Forecast evaluation for data scientists: common pitfalls and best practices},
  author={Hewamalage, Hansika and Ackermann, Klaus and Bergmeir, Christoph},
  journal={Data Mining and Knowledge Discovery},
  volume={37},
  number={2},
  pages={788--832},
  year={2023},
  publisher={Springer},
  doi={10.1007/s10618-022-00894-5}
}

@book{otext,
    title = "Forecasting: principles and practice, 3nd edition",
    author = "Hyndman, R.J. \& Athanasopoulos, G.",
    year = "2018", 
    number = {URL: OTexts.com/fpp3}
}
@misc{akiba2019optuna,
      title={Optuna: A Next-generation Hyperparameter Optimization Framework}, 
      author={Takuya Akiba and Shotaro Sano and Toshihiko Yanase and Takeru Ohta and Masanori Koyama},
      year={2019},
      eprint={1907.10902},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@article{deamorim2023scaling,
  title={The choice of scaling technique matters for classification performance},
  author={de Amorim, Lucas B.V. and Mirandola, Denis and Monard, Maria Carolina},
  journal={Applied Soft Computing},
  volume={133},
  pages={109918},
  year={2023},
  publisher={Elsevier},
  doi={10.1016/j.asoc.2022.109924}
}













@misc{chatgpt,
  author = {{OpenAI}},
  title = {ChatGPT: Optimizing Language Models for Dialogue.},
  year = {2022},
  howpublished = {\url{https://openai.com/blog/chatgpt}},
  note = {Accessed: 2025-02-23}
}

@misc{copilot,
  author = {{Friedman, Nat.}},
  title = {Introducing GitHub Copilot: your AI pair programmer.},
  year = {2021},
  howpublished = {\url{https://copilot.github.com/}},
  note = {Accessed: 2025-02-23}
}

@manual{pytorch2025docs,
  title        = {PyTorch Documentation},
  author       = {{PyTorch Contributors}},
  organization = {PyTorch},
  year         = {2025},
  url          = {https://docs.pytorch.org/docs/stable/index.html},
  note         = {Accessed: 2025-05-30}
}

@manual{scikit-learn-docs,
  title        = {scikit-learn: Machine Learning in Python — Documentation},
  author       = {{scikit-learn developers}},
  organization = {scikit-learn},
  year         = {2025},
  url          = {https://scikit-learn.org/stable/documentation.html},
  note         = {Accessed: 2025-05-30}
}

@misc{researchrabbit2025,
  author       = {{ResearchRabbit}},
  title        = {ResearchRabbit: AI-Powered Literature Discovery},
  year         = {2025},
  url          = {https://www.researchrabbit.ai},
  note         = {Accessed: 2025-05-30}
}

@misc{grammarly,
  author = {{Grammarly}},
  title = {Grammarly: Free AI Writing Assistance.},
  year = {2025},
  howpublished = {\url{https://app.grammarly.com/}},
  note = {Accessed: 2025-06-05}
}

==> Content/7._Results_and_Discussion/tables/pre_tables.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DATA PIPELINE RESULT  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%  DRIFT RESULT + ALL %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[h]
    \centering
    \caption{WF Id 15 WT Id 108 drift results for multiple ML models.}
    \label{tab:model_performance}
    \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
        \textbf{Model} & \textbf{Year} & \textbf{$R_1$ delta} & \textbf{$R_2$ delta} & \textbf{Drift} & \textbf{MAPE} & \textbf{T year} \\ \hline
        MLPRegressor & 2019 & 6,288  &          &        & 11,724 & 2018 \\ \hline
        MLPRegressor & 2020 & 6,288  & 9,9142   & 3,627  & 15,042 & 2018 \\ \hline
        MLPRegressor & 2021 & 6,288  & 8,7142   & 2,427  & 14,131 & 2018 \\ \hline
        MLPRegressor & 2022 & 6,288  & 17,017   & 10,729 & 22,150 & 2018 \\ \hline
        MLPRegressor & 2023 & 6,288  & 21,002   & 14,714 & 25,418 & 2018 \\ \hline
        RFRegressor  & 2019 & 0,885  &          &        & 6,210  & 2018 \\ \hline
        RFRegressor  & 2020 & 0,885  & 4,457    & 3,572  & 7,431  & 2018 \\ \hline
        RFRegressor  & 2021 & 0,885  & 7,412    & 6,527  & 10,281 & 2018 \\ \hline
        RFRegressor  & 2022 & 0,885  & 14,355   & 13,469 & 16,261 & 2018 \\ \hline
        RFRegressor  & 2023 & 0,885  & 20,130   & 19,244 & 21,265 & 2018 \\ \hline
        XGBRegressor & 2019 & -0,180 &          &        & 5,210  & 2018 \\ \hline
        XGBRegressor & 2020 & -0,180 & 2,153    & 2,332  & 6,003  & 2018 \\ \hline
        XGBRegressor & 2021 & -0,180 & 4,896    & 5,076  & 8,201  & 2018 \\ \hline
        XGBRegressor & 2022 & -0,180 & 11,230   & 11,409 & 13,738 & 2018 \\ \hline
        XGBRegressor & 2023 & -0,180 & 16,660   & 16,843 & 18,650 & 2018 \\ \hline
        KNNRegressor & 2019 & -0,620 &          &        & 5,406  & 2018 \\ \hline
        KNNRegressor & 2020 & -0,620 & 0,388    & 1,008  & 5,567  & 2018 \\ \hline
        KNNRegressor & 2021 & -0,620 & 1,668    & 2,288  & 6,191  & 2018 \\ \hline
        KNNRegressor & 2022 & -0,620 & 6,781    & 7,401  & 9,366  & 2018 \\ \hline
        KNNRegressor & 2023 & -0,620 & 9,732    & 10,352 & 11,957 & 2018 \\ \hline
    \end{tabular}
\end{table*}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%  DRIFT RESULT + ALL %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[h]
    \centering
    \caption{WF Id 12 WT Id 80 drift results for multiple ML models.}
    \label{tab:model_performance}
    \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
        \textbf{Model} & \textbf{Year} &\textbf{ $R_1$ delta} & \textbf{$R_2$ delta} & \textbf{Drift} & \textbf{MAPE} & \textbf{T year} \\ \hline
        MLPRegressor & 2019 & -6,127  &          &          & 13,021 & 2018 \\ \hline
        MLPRegressor & 2020 & -6,127  & -8,098   & -1,971   & 14,870 & 2018 \\ \hline
        MLPRegressor & 2021 & -6,127  & -19,811  & -13,684  & 26,340 & 2018 \\ \hline
        MLPRegressor & 2022 & -6,127  & -12,261  & -6,133   & 20,045 & 2018 \\ \hline
        MLPRegressor & 2023 & -6,127  & -10,709  & -4,582   & 16,922 & 2018 \\ \hline
        RFRegressor  & 2019 & -1,613  &          &          & 5,723  & 2018 \\ \hline
        RFRegressor  & 2020 & -1,613  & -5,316   & -3,702   & 8,536  & 2018 \\ \hline
        RFRegressor  & 2021 & -1,613  & -12,828  & -11,214  & 16,042 & 2018 \\ \hline
        RFRegressor  & 2022 & -1,613  & -10,327  & -8,713   & 13,505 & 2018 \\ \hline
        RFRegressor  & 2023 & -1,613  & -8,310   & -6,697   & 11,372 & 2018 \\ \hline
        XGBRegressor & 2019 & -1,759  &          &          & 5,867  & 2018 \\ \hline
        XGBRegressor & 2020 & -1,759  & -4,900   & -3,141   & 8,568  & 2018 \\ \hline
        XGBRegressor & 2021 & -1,759  & -12,590  & -10,831  & 16,115 & 2018 \\ \hline
        XGBRegressor & 2022 & -1,759  & -9,335   & -7,576   & 12,840 & 2018 \\ \hline
        XGBRegressor & 2023 & -1,759  & -7,883   & -6,124   & 11,167 & 2018 \\ \hline
        KNNRegressor & 2019 & -0,407  &          &          & 5,878  & 2018 \\ \hline
        KNNRegressor & 2020 & -0,407  & -3,186   & -2,778   & 7,715  & 2018 \\ \hline
        KNNRegressor & 2021 & -0,407  & -11,548  & -11,141  & 15,491 & 2018 \\ \hline
        KNNRegressor & 2022 & -0,407  & -7,843   & -7,436   & 12,257 & 2018 \\ \hline
        KNNRegressor & 2023 & -0,407  & -6,662   & -6,255   & 10,498 & 2018 \\ \hline
    \end{tabular}                       
\end{table*}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%  DRIFT RESULT + ALL %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[h]
    \centering
    \caption{WF Id 1 WT Id 7 drift results for multiple ML models.}
    \label{tab:model_performance}
    \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
        \textbf{Model} & \textbf{Year} & \textbf{$R_1$ delta} & \textbf{$R_2$ delta} & \textbf{Drift} & \textbf{MAPE} & \textbf{T year} \\ \hline
        MLPRegressor & 2019 & 11,613 &          &        & 13,359 & 2018 \\ \hline
        MLPRegressor & 2020 & 11,613 & 11,747   & 0,134  & 13,398 & 2018 \\ \hline
        MLPRegressor & 2021 & 11,613 & 10,220   & -1,393 & 12,645 & 2018 \\ \hline
        MLPRegressor & 2022 & 11,613 & 10,600   & -1,014 & 12,672 & 2018 \\ \hline
        MLPRegressor & 2023 & 11,613 & 8,678    & -2,935 & 11,833 & 2018 \\ \hline
        RFRegressor  & 2019 & 4,207  &          &        & 6,967  & 2018 \\ \hline
        RFRegressor  & 2020 & 4,207  & 9,095    & 4,888  & 9,838  & 2018 \\ \hline
        RFRegressor  & 2021 & 4,207  & 8,558    & 4,351  & 9,180  & 2018 \\ \hline
        RFRegressor  & 2022 & 4,207  & 8,396    & 4,189  & 8,782  & 2018 \\ \hline
        RFRegressor  & 2023 & 4,207  & 7,025    & 2,818  & 8,210  & 2018 \\ \hline
        XGBRegressor & 2019 & 6,176  &          &        & 7,539  & 2018 \\ \hline
        XGBRegressor & 2020 & 6,176  & 7,864    & 1,688  & 8,563  & 2018 \\ \hline
        XGBRegressor & 2021 & 6,176  & 7,432    & 1,257  & 8,102  & 2018 \\ \hline
        XGBRegressor & 2022 & 6,176  & 6,854    & 0,678  & 7,567  & 2018 \\ \hline
        XGBRegressor & 2023 & 6,176  & 5,034    & -1,142 & 6,870  & 2018 \\ \hline
        KNNRegressor & 2019 & 7,110  &          &        & 8,259  & 2018 \\ \hline
        KNNRegressor & 2020 & 7,110  & 7,316    & 0,206  & 8,276  & 2018 \\ \hline
        KNNRegressor & 2021 & 7,110  & 6,748    & -0,362 & 7,736  & 2018 \\ \hline
        KNNRegressor & 2022 & 7,110  & 5,593    & -1,517 & 7,068  & 2018 \\ \hline
        KNNRegressor & 2023 & 7,110  & 3,146    & -3,964 & 6,604  & 2018 \\ \hline
    \end{tabular}
\end{table*}




















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%  DRIFT RESULT + WS-AT  %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[h]
    \centering
    \caption{WF Id 15 WT Id 108 drift results for multiple ML models restricted to WindSpeed and AmbTemp.}
    \label{tab:model_performance}
    \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
        \textbf{Model} & \textbf{Year} & \textbf{$R_1$ delta} & \textbf{$R_2$ delta} & \textbf{Drift} & \textbf{MAPE} & \textbf{T year} \\ \hline
        MLPRegressor & 2019 & -5,593  &          &         & 14,511 & 2018 \\ \hline
        MLPRegressor & 2020 & -5,593  & -6,363   & -0,770  & 13,656 & 2018 \\ \hline
        MLPRegressor & 2021 & -5,593  & -9,659   & -4,066  & 18,187 & 2018 \\ \hline
        MLPRegressor & 2022 & -5,593  & -10,816  & -5,223  & 17,600 & 2018 \\ \hline
        MLPRegressor & 2023 & -5,593  & -18,455  & -12,862 & 23,248 & 2018 \\ \hline
        RFRegressor  & 2019 & -11,529 &          &         & 19,676 & 2018 \\ \hline
        RFRegressor  & 2020 & -11,529 & -14,685  & -3,156  & 20,907 & 2018 \\ \hline
        RFRegressor  & 2021 & -11,529 & -15,136  & -3,607  & 21,941 & 2018 \\ \hline
        RFRegressor  & 2022 & -11,529 & -17,340  & -5,812  & 23,291 & 2018 \\ \hline
        RFRegressor  & 2023 & -11,529 & -22,899  & -11,371 & 28,310 & 2018 \\ \hline
        XGBRegressor & 2019 & -11,422 &          &         & 19,975 & 2018 \\ \hline
        XGBRegressor & 2020 & -11,422 & -14,624  & -3,202  & 20,856 & 2018 \\ \hline
        XGBRegressor & 2021 & -11,422 & -14,986  & -3,564  & 21,942 & 2018 \\ \hline
        XGBRegressor & 2022 & -11,422 & -17,080  & -5,658  & 23,171 & 2018 \\ \hline
        XGBRegressor & 2023 & -11,422 & -22,677  & -11,255 & 28,191 & 2018 \\ \hline
        KNNRegressor & 2019 & -11,459 &          &         & 19,815 & 2018 \\ \hline
        KNNRegressor & 2020 & -11,459 & -14,579  & -3,120  & 20,992 & 2018 \\ \hline
        KNNRegressor & 2021 & -11,459 & -15,022  & -3,563  & 22,074 & 2018 \\ \hline
        KNNRegressor & 2022 & -11,459 & -17,368  & -5,909  & 23,479 & 2018 \\ \hline
        KNNRegressor & 2023 & -11,459 & -23,054  & -11,595 & 28,594 & 2018 \\ \hline
    \end{tabular}
\end{table*}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%  DRIFT RESULT + WS-AT  %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[h]
    \centering
    \caption{WF Id 12 WT Id 80 drift results for multiple ML models restricted to WindSpeed and AmbTemp.}
    \label{tab:model_performance}
    \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
        \textbf{Model} & \textbf{Year} & \textbf{$R_1$ delta} & \textbf{$R_2$ delta} & \textbf{Drift} & \textbf{MAPE} & \textbf{T year} \\ \hline
        MLPRegressor & 2019 & 0,275  &         &         & 8,620  & 2018 \\ \hline
        MLPRegressor & 2020 & 0,275  & -2,110  & -2,384  & 10,666  & 2018 \\ \hline
        MLPRegressor & 2021 & 0,275  & -11,609 & -11,884 & 17,501  & 2018 \\ \hline
        MLPRegressor & 2022 & 0,275  & -10,091 & -10,366 & 16,130  & 2018 \\ \hline
        MLPRegressor & 2023 & 0,275  & -7,437  & -7,712  & 14,006  & 2018 \\ \hline
        RFRegressor  & 2019 & 0,385  &         &         & 6,873  & 2018 \\ \hline
        RFRegressor  & 2020 & 0,385  & -2,461  & -2,845  & 9,100  & 2018 \\ \hline
        RFRegressor  & 2021 & 0,385  & -10,852 & -11,237 & 14,590  & 2018 \\ \hline
        RFRegressor  & 2022 & 0,385  & -10,426 & -10,811 & 14,299  & 2018 \\ \hline
        RFRegressor  & 2023 & 0,385  & -8,195  & -8,580  & 12,342  & 2018 \\ \hline
        XGBRegressor & 2019 & 0,143  &         &         & 7,169  & 2018 \\ \hline
        XGBRegressor & 2020 & 0,143  & -2,739  & -2,882  & 9,432  & 2018 \\ \hline
        XGBRegressor & 2021 & 0,143  & -11,038 & -11,181 & 14,953  & 2018 \\ \hline
        XGBRegressor & 2022 & 0,143  & -10,704 & -10,847 & 14,603  & 2018 \\ \hline
        XGBRegressor & 2023 & 0,143  & -8,360  & -8,503  & 12,609  & 2018 \\ \hline
        KNNRegressor & 2019 & 0,217  &         &         & 7,057  & 2018 \\ \hline
        KNNRegressor & 2020 & 0,217  & -2,576  & -2,793  & 9,289  & 2018 \\ \hline
        KNNRegressor & 2021 & 0,217  & -10,894 & -11,111 & 14,777  & 2018 \\ \hline
        KNNRegressor & 2022 & 0,217  & -10,456 & -10,673 & 14,475  & 2018 \\ \hline
        KNNRegressor & 2023 & 0,217  & -8,130  & -8,347  & 12,482  & 2018 \\ \hline
    \end{tabular}                       
\end{table*}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%  DRIFT RESULT + WS-AT  %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[h]
    \centering
    \caption{WF Id 1 WT Id 7 drift results for multiple ML models restricted to WindSpeed and AmbTemp.}
    \label{tab:model_performance}
    \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
        \textbf{Model} & \textbf{Year} & \textbf{$R_1$ delta} & \textbf{$R_2$ delta} & \textbf{Drift} & \textbf{MAPE} & \textbf{T year} \\ \hline
        MLPRegressor & 2019 & 5,161  &          &         & 9,690        & 2018 \\ \hline
        MLPRegressor & 2020 & 5,161  & 6,344    & 1,184   & 9,600        & 2018 \\ \hline
        MLPRegressor & 2021 & 5,161  & 4,740    & -0,421  & 9,550        & 2018 \\ \hline
        MLPRegressor & 2022 & 5,161  & 4,190    & -0,971  & 8,930        & 2018 \\ \hline
        MLPRegressor & 2023 & 5,161  & -0,862   & -6,023  & 10,454        & 2018 \\ \hline
        RFRegressor  & 2019 & 0,402  &          &         & 7,349        & 2018 \\ \hline
        RFRegressor  & 2020 & 0,402  & 1,346    & 0,944   & 6,826        & 2018 \\ \hline
        RFRegressor  & 2021 & 0,402  & 0,720    & 0,318   & 6,692        & 2018 \\ \hline
        RFRegressor  & 2022 & 0,402  & -1,516   & -1,918  & 6,793        & 2018 \\ \hline
        RFRegressor  & 2023 & 0,402  & -6,651   & -7,053  & 10,254        & 2018 \\ \hline
        XGBRegressor & 2019 & 0,369  &          &         & 7,384        & 2018 \\ \hline
        XGBRegressor & 2020 & 0,369  & 1,371    & 1,001   & 6,890        & 2018 \\ \hline
        XGBRegressor & 2021 & 0,369  & 0,682    & 0,313   & 6,825        & 2018 \\ \hline
        XGBRegressor & 2022 & 0,369  & -1,583   & -1,952  & 6,979        & 2018 \\ \hline
        XGBRegressor & 2023 & 0,369  & -6,767   & -7,136  & 10,439        & 2018 \\ \hline
        KNNRegressor & 2019 & 0,695  &          &         & 7,541        & 2018 \\ \hline
        KNNRegressor & 2020 & 0,695  & 1,627    & 0,932   & 7,071        & 2018 \\ \hline
        KNNRegressor & 2021 & 0,695  & 0,881    & 0,186   & 6,898        & 2018 \\ \hline
        KNNRegressor & 2022 & 0,695  & -1,314   & -2,009  & 7,089        & 2018 \\ \hline
        KNNRegressor & 2023 & 0,695  & -6,432   & -7,127  & 10,415        & 2018 \\ \hline
    \end{tabular}
\end{table*}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%  Sensitivity + ALL    %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[h]
    \centering
    \caption{WF Id 1 WT Id 7 sensitivity results for multiple ML models.}
    \label{tab:model_performance}
    \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
        \textbf{Model} & \textbf{Year} & \textbf{Drift} & \textbf{MAPE} & \textbf{T year} \\ \hline
        MLPRegressor &      & -3,041 & 7,063   & 2018 \\ \hline
        MLPRegressor & 2019 & 3,760  & 6,937   & 2018 \\ \hline
        MLPRegressor & 2020 & 3,725  & 6,752   & 2018 \\ \hline
        MLPRegressor & 2021 & 2,917  & 6,237   & 2018 \\ \hline
        MLPRegressor & 2022 & 1,747  & 6,190   & 2018 \\ \hline
        MLPRegressor & 2023 & -0,528 & 6,722   & 2018 \\ \hline
        RFRegressor  &      & -0,104 & 2,835   & 2018 \\ \hline
        RFRegressor  & 2019 & 3,177  & 5,361   & 2018 \\ \hline
        RFRegressor  & 2020 & 8,374  & 9,142   & 2018 \\ \hline
        RFRegressor  & 2021 & 7,587  & 8,252   & 2018 \\ \hline
        RFRegressor  & 2022 & 6,245  & 7,146   & 2018 \\ \hline
        RFRegressor  & 2023 & 4,363  & 6,338   & 2018 \\ \hline
        XGBRegressor &      & -0,026 & 3,664   & 2018 \\ \hline
        XGBRegressor & 2019 & 5,784  & 6,842   & 2018 \\ \hline
        XGBRegressor & 2020 & 8,050  & 8,578   & 2018 \\ \hline
        XGBRegressor & 2021 & 7,586  & 8,149   & 2018 \\ \hline
        XGBRegressor & 2022 & 6,847  & 7,349   & 2018 \\ \hline
        XGBRegressor & 2023 & 5,777  & 6,719   & 2018 \\ \hline
        KNNRegressor &      & 0,045  & 5,112   & 2018 \\ \hline
        KNNRegressor & 2019 & 6,978  & 8,100   & 2018 \\ \hline
        KNNRegressor & 2020 & 7,291  & 8,248   & 2018 \\ \hline
        KNNRegressor & 2021 & 6,716  & 7,707   & 2018 \\ \hline
        KNNRegressor & 2022 & 5,564  & 7,055   & 2018 \\ \hline
        KNNRegressor & 2023 & 3,121  & 6,605   & 2018 \\ \hline
    \end{tabular}
\end{table*}









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%  Sensitivity + WS&AT   %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[h]
    \centering
    \caption{WF Id 1 WT Id 7 sensitivity results for multiple ML models restricted to WindSpeed and AmbTemp.}
    \label{tab:model_performance}
    \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
        \textbf{Model}        & \textbf{Year} & \textbf{Drift}  & \textbf{MAPE}     & \textbf{T year} \\ \hline
        MLPRegressor &      & 10,135 & 16,337   & 2018 \\ \hline
        MLPRegressor & 2019 & 10,098 & 16,314   & 2018 \\ \hline
        MLPRegressor & 2020 & 10,892 & 15,964   & 2018 \\ \hline
        MLPRegressor & 2021 & 11,058 & 17,170   & 2018 \\ \hline
        MLPRegressor & 2022 & 8,343  & 14,707   & 2018 \\ \hline
        MLPRegressor & 2023 & 3,425  & 14,069   & 2018 \\ \hline
        RFRegressor  &      & -0,056 & 7,246    & 2018 \\ \hline
        RFRegressor  & 2019 & 0,325  & 7,184    & 2018 \\ \hline
        RFRegressor  & 2020 & 1,308  & 6,702    & 2018 \\ \hline
        RFRegressor  & 2021 & 0,627  & 6,522    & 2018 \\ \hline
        RFRegressor  & 2022 & -1,633 & 6,771    & 2018 \\ \hline
        RFRegressor  & 2023 & -6,784 & 10,315   & 2018 \\ \hline
        XGBRegressor &      & 0,000  & 7,562    & 2018 \\ \hline
        XGBRegressor & 2019 & 0,412  & 7,242    & 2018 \\ \hline
        XGBRegressor & 2020 & 1,466  & 6,855    & 2018 \\ \hline
        XGBRegressor & 2021 & 0,694  & 6,690    & 2018 \\ \hline
        XGBRegressor & 2022 & -1,638 & 7,002    & 2018 \\ \hline
        XGBRegressor & 2023 & -6,784 & 10,566   & 2018 \\ \hline
        KNNRegressor &      & 0,331  & 7,258    & 2018 \\ \hline
        KNNRegressor & 2019 & 0,747  & 7,698    & 2018 \\ \hline
        KNNRegressor & 2020 & 1,708  & 7,225    & 2018 \\ \hline
        KNNRegressor & 2021 & 0,919  & 7,010    & 2018 \\ \hline
        KNNRegressor & 2022 & -1,357 & 7,196    & 2018 \\ \hline
        KNNRegressor & 2023 & -6,407 & 10,447   & 2018 \\ \hline
    \end{tabular}    
\end{table*}
